Assessing the Difficulty of Classifying ConceptNet Relations in a Multi-Label Classification Setting

Commonsense knowledge relations are crucial for advanced NLU tasks. We examine the learnability of such relations as represented in CONCEPTNET, taking into account their specific properties, which can make relation classification difficult: a given concept pair can be linked by multiple relation types, and relations can have multi-word arguments of diverse semantic types. We explore a neural open world multi-label classification approach that focuses on the evaluation of classification accuracy for individual relations. Based on an in-depth study of the specific properties of the CONCEPTNET resource, we investigate the impact of different relation representations and model variations. Our analysis reveals that the complexity of argument types and relation ambiguity are the most important challenges to address. We design a customized evaluation method to address the incompleteness of the resource that can be expanded in future work.

==> CN.tex <==
\section{The Difficulty of ConceptNet Relation Classification}

\af{[there is nothing inherently new here, Table 1 is not taken into account, no hypotheses are stated as to the classification difficulty and results, this is not yet a very useful section (but costs half a page)]}\rednote{MB: I agree. I moved 3.1 (CN Resource and Dataset) to the beginning of the next section. 3.2 only summarizes stuff we mention before and later, so this can be ommited completely.}


\subsection{\cn~Resource and Dataset}\label{sec:data}
%%MB: moved to next section
In response to the difficulties of automatic acquisition of CS knowledge, the Open Mind Common Sense project \cite{singh2002} created \cn, %\footnote{\url{http://conceptnet.io/}}
a knowledge base gathered from volunteer contributions over the web, to which were later added expert-created resources (such as WordNet) and knowledge obtained through games with a purpose \cite{SPEER12.1072.L12-1639}. 
The current version, \cn~5.6, comprises 37 relations, some of which are commonly used in other resources like WordNet (e.g.\ \rel{IsA, PartOf}) while most others are more specific to capturing commonsense information and as such are particular to \cn~ (e.g.\ \rel{HasPrerequisite} or \rel{MotivatedByGoal}). With only very few exceptions (such as \rel{Synonym} or \rel{Antonym}), CN-relations are asymmetric. % (see \textit{Supplement}). 
The English version consists of 1.9 million concepts and 1.1 million links to other databases like DBpedia. 

\subsection{Specific Properties of \cn}

Given its crowd-sourced nature, \cn~contains facts of varying quality, and biases reflecting knowledge or intentions of the contributors. But, as mentioned in the introduction,
%Furthermore, 
\cn~features further
%certain other 
characteristics that can make relation classification difficult:
%(cf.\ Section \ref{sec:intro}): 
%There might be 
several %possible 
distinct
relation types may hold for a given concept pair; some relation types overlap at the type level; and some relations are not clearly enough defined and thus  relation instances can be inhomogeneous. \af{in most relation dataset we have argument types that overlap, so why is this a specific property of CN? -- include MWE arguments instead}
Yet, one of the most striking properties of \cn~is the ambiguity of the relation set. Relation inventories for specific tasks or datasets are usually designed to be disjunct, since the goal is to have only one possible relation for each instance \cite{nastase2013semantic}. The relations in \cn~ do not conform to this, as we observe  interconnections between relation types. Some relations such as \rel{UsedFor} and \rel{CapableOf} seem to be inferentially related -- {\em if c$_1$ is \rel{capable of} achieving an action c$_2$, $c_1$ can be \rel{used for} performing $c_2$}, as for pairs $\langle$\textit{forklifts},\textit{lift heavy things}$\rangle$. \cn~ also contains relations that are clearly ambiguous such as \textsc{HasSubevent} and \textsc{HasPrerequisite}. Relation overlap can also be coincidental rather than implied: pairs like $\langle$\textit{children,throw things}$\rangle$ can be found in the relations \rel{Desires} and \rel{CapableOf}, and $\langle$\textit{walking in the rain,get wet}$\rangle$ can be connected both with \rel{HasSubevent} and \rel{Causes}.
%noisy. \\
%OLD:(i) relation arguments can be verbal or nominal \textit{multi-word phrases} covering various entity types (location, entities, properties, events or states); (ii) many \cn~relations are tightly interconnected, which places their instances in close vicinity in semantic space; (iii) some relation types are ambiguous or overlapping at the type level, such as \rel{HasSubevent} and \rel{HasPrerequisite} (e.g., \textit{learning} is a \rel{Subevent} of \textit{taking an exam} but also a \rel{Prerequisite}); (iv) some relations are even vaguely defined and thus noisy, for instance \rel{IsA} or \rel{HasProperty} -- well-known relations from other resources -- for which we find instances such as: \tr{car}{IsA}{people mover}, \tr{car}{IsA}{an object with high cost}. These are effects of the crowd-sourcing nature of \cn. They should be instances of \rel{UsedFor} and \rel{HasProperty}, respectively.

%\subsection{Relation Ambiguities in \cn} 

%In table \ref{table:examples} we list more cases of ambiguous relations we found in \cn.

%This challenge is evidenced by the TSNE plot in Fig.\ref{fig:semevalclusters} which is a visualization of %a few 
%instances from the relation inventory. There is no clear separation or clustering of instances that represent the same relation type.




==> applications.tex <==
%\subsection{\cn~ Knowledge Used in Applications}
\subsection{Using \cn~ in Applications}
\label{sec:related-applications}
%In recent years, 
\cn~has
%as the resource of choice to provide CS knowledge, 
been put to use in
%adopted to provide needed information for 
many advanced NLU tasks.
\citet{speer17} 
%utilize the graph-structured knowledge in \cn~ to 
built concept embeddings called 
\textit{Numberbatch}
%semantic spaces 
from \cn~that are supposed to be more informative than purely distributional word embeddings.\footnote{This situation has changed with the recent BERT word embeddings. \af{TODO: explicate, add REF}} %alone.
They use retrofitting methods \cite{Faruqui14} for
combining the information contained in \textit{Glove} and \textit{word2vec} embeddings with the pruned \cn~graph to form a hybrid semantic space. 
%\citet{speer17} call
%The resulting 
%is a labeled matrix of 
%word embeddings are called
%Which they call 
%\textit{\cn~Numberbatch}
They %find
 show that \textit{Numberbatch} embeddings 
% and are shown to 
 perform significantly better than other embeddings when 
%being 
applied to a
%the 
\textit{word relatedness task}
%where the model has to rank the relatedness of pairs of words, as well as on 
or to predicting missing values
in 
%other downstream tasks such as \textit{analogies}, where the model has to predict
%fill in 
%missing values 
%of a proportional 
in \textit{analogies} of the form \textit{a$_1$ is to b$_1$ what a$_2$ is to b$_2$}. \\
\cn~is also being used as database for downstream tasks, sometimes using specific relations \cite{8046084}, sometimes using graph similarity metrics \cite{Adi18}. 
\citet{weissenborn2018} 
%for example introduce an architecture for 
integrating knowledge from 
%and Wikipedia 
\cn~in two NLU-tasks: document question answering and  recognizing textual entailment. 
They encode knowledge from \cn~in the form of simple linguistic statements, which are processed by their neural model in addition to the task-specific documents. In this way they obtain knowledge-enriched text representations that make even simple model architectures competitive with complex SOTA models.
%As input for their neural model, they %replace static word embeddings with 
%use embeddings which are functions of the task inputs and \cn~and Wikipedia as background knowledge. %in the form of freetext statements. 
%Their results show that using these refined embedding improves nerual NLU models, and that even very simple task architectures (such as simple BiLSTM readers) can become competitive with state of the art, task-specific architectures when augmented with knowledge-enhanced embeddings.\\
The SemEval-2018 Task 11 \textit{Machine Comprehension Using Commonsense Knowledge} \cite{semeval18-11} 
%was designed to 
evaluates how well systems are capable of 
%correctly 
answering questions that may involve commonsense knowledge, casting the task in a multiple choice QA setting. 
Participating models had to find the best answer for multiple choice questions based on narrative text by including commonsense knowledge from sources of their choice. 
%Surprisingly, 
\cn~was employed by 2 of 11 participating models, which ranked 1st and 5th in the evaluation.
The winning system,  \citet{Wang2018}, 
%one of them \cite{Wang2018} 
%two models using \cn~, was 
%succeeded as the best performing system. They 
represents text, question, and answers by combining GloVe embeddings, part-of-speech labels, named entity tags and relation embeddings learned on \cn.  
Relation embeddings. These embeddings are randomly initialized and determined by querying ConceptNet
whether there is an edge between words or phrases in the given text and the question or answer. All 37 \cn~ relations were considered.
%\af{selected or all relations? method used for relation learning?}
These representations are used as input to an neural architecture with attention. They achieve an accuracy of 84\%, outperforming the baselines by a large margin.
The other system, \citet{Gonzalez18}, use ConceptNet in form of pretrained \textit{Numberbatch} embeddings. %which encode information from ConceptNet, as described above.
They employ a BiLSTM with attention to model interactions between the text, question and answers, and encode each word
with
%and represent each word based on 
\textit{Numberbatch} embeddings, achieving
%. They achieve 
an accuracy of 75\%.
%and are ranked as the fifth best performing system.

Downstream applications that successfully employ  knowledge from \cn~include vision \cite{Le13}, %question answering \cite{1712.00733,8046084}, 
reading comprehension \cite{mihaylovfrank:2018,1712.00733} or dialogue modeling \cite{Young2018Augmenting}.
%, just to name a few.
%However, to our knowledge none of the systems deploying \cn~take into account the multi-label structure of this resource. In the next paragraph, we will therefore have a closer look at multi-label classification approaches and how we can adapt them to \cn~relation classification. \af{The multi-label characteristics is mostly an issue for evaluation, therefore it should be mentioned when discussing how to learn such relations and how to evaluate the results. Eg. Weissenborn does not need to care: he just takes what he finds in CN (or Numberbatch) as static resources.}
 
%\subsection{Multi-Label Classification Approaches}
%\rednote{TBD.}
% ELIMINATED (AF)

%ConceptNet Numberbatch consists of state-of-the-art semantic vectors (also known as word embeddings) that can be used directly as a representation of word meanings or as a starting point for further machine learning.
%We have compared word embeddings that represent only distributional semantics (word2vec, GloVe, and LexVec), word embeddings that represent only relational knowledge (ConceptNet PPMI), and the combination of the two (ConceptNet Numberbatch), and we have shown that the whole is more than the sum of its parts.

==> conclusion_old.tex <==
- In light of these challenges posed by the specific properties of \cn, we perform an in-depth study on learning CS relations as captured in this resource. 
improvement of our \textsc{Ffnn} model when enhanced with \textsc{Rnn} for multiword representation (Open world-one class setting; in percentage points) (column 7)
- As mentioned before, one specific characteristic of \cn~ is that there might be multiple possible labels (relations) for one concept pair which are not mutually exclusive (cf. Section \ref{sec:multimodel}) -- other than disjunct relation inventories with only one possible relation for each instance (for example the \citeauthor{hendrickx-EtAl:2010:SemEval} \citeyear{hendrickx-EtAl:2010:SemEval}). 

Outlook: ?
 -We determine which approaches and representations are best suited for \cns~based commonsense relation classification.
We investigated challenges of relation classification for commonsense knowledge relations 
based on \cn.
%, as opposed to semantic relations used in
%classification 
%other sources, such as SemEval-2010 Task8. 
Using a subset of high-quality relation instances from \cn, we analyze the difficulty of classifying these relations in a
%performance of relation classification in a 
multi-class setting. We apply learning frameworks built on
%combined with 
%models by building various models that combine 
word embeddings
%with learning frameworks 
ranging from clustering to linear SVM and deep learning models. 
We also apply graph embedding methods that exploit the structure of the network with small and extended training data.
%Besides approaching this task from the perspective of classical relation classification, we additionally perform relation classification by experimenting with link prediction methods on the Li et al. (2016) dataset using factorization algorithms that exploit the structure of this graph.
Models using RNNs for representing arguments yield best results. SVM and FFNN models based on these representations show complementarity performance on relations depending on their multiword characteristics. 
%feeding embedding representations which concatenate related terms into Feed Forward Neural Network Architectures which we then enhance with a RNN for generating representation for multiword terms are best suited for learning commonsense relations, 
But both model types achieve high scores of 73 and 75 F1 scores 
%for 10 relations 
using only representations of argument pairs.
%We investigate the performance of our models for the relations respectively and find that 
%our models perform best for the relation \textsc{AtLocation}, while \textsc{HasSubevent} is a relation that seems to be hard to classify. 
%analyze the distinctiveness of the relation set
%commonsense relations and 
We find that many relations in CN are inferentially related or ambiguous, which makes them hard to distinguish.
%for our models. 
%Another specific challenges posed by the CONCEPTNET is that most of the concepts are represented as multi-word terms.  
Also, graph embedding models are confronted with severe challenges and perform worse compared to SVM and FFNN due to the sparsity of the \cn~graph in its current form.
%TOO STRONG: This suggests that graph embedding models maybe unsuitable to common sense relation classification task, especially when large scale data sets are not available.
%\rednote{results on SemEval 2010-8 - todo}
In future work, we will further study how to address
%characteristics of 
multiword terms in \cns~and ways of ensuring higher connectivity in spite of this challenge. 
%\rednote{keep the following or close here?}
%focus on enhancing our systems with negative sampling methods and \rednote{..., tbd}. Based on our approach and the observations presented in this paper, we want to work towards commonsense knowledge acquisition and targeted information extraction from natural language text.
%The multiword character of the relation set is thus a specific challenge.




\begin{itemize}
\item collect important insights from analysis 

\item Open world, so model can be applied to open data to learn new related word pairs 
\item Phrase Splitting, Granularity of Concepts
\item Prospects, future work
\end{itemize}

%We find that applying vector offsets to capture semantic relationships (Vylomova et al. 2016) works reasonably well for commonsense classification: In our experiments, we achieve ... \\

Future Work: CS Know. Acquisition,Targeted IE 

Closing: Systems capable of reliably performing commonsense relation classification can be embedded into different types of knowledge acquisition systems and therefore help in overcoming the knowledge acquisition bottleneck. For example, commonsense relation classification approaches can be used to find the relations between newly acquired term pairs that are known to be semantically related. This process results in knowledge acquisition as the term pairs and their predicted relations can be seen as formerly unknown knowledge facts.

\begin{figure*}[t]

%\begin{subfigure}{.6\textwidth}
\centering
\includegraphics[scale=0.7]{png/dis_new.png}
%\includegraphics[width=0.35\textwidth]{png/mwt.png}
\caption{Number of instances per 14 most frequent relations in  \textsc{Cn-Omcs-Cln}.}
\label{fig:distributions}
%\end{subfigure}
%~
%\begin{subfigure}{.4\textwidth}
%\centering
%\includegraphics[width=\textwidth]{png/other.png}
%\includegraphics[scale=0.7]{png/results_new_2.png}
%\caption{Relations contained in the \rel{Other} class.} %on \textit{CN\_10\_1400}}
%\label{fig:other}
%\end{subfigure}
~
%\caption{Relations in \cn: 14 most frequent relations} %+ relations contained in \textsc{Other}.}
\label{fig:distributions+other}
\end{figure*}

==> tables/amigrelations.tex <==
\begin{table} [t]
\centering
\small{
\begin{tabular}{lll}
Co-occurring Relations & \textsc{Cn-Om-} & \textsc{Cn-Om-}%& Examples 
\\
 & \textsc{cs-Cln} & \textsc{cs-14}\\
\hline
\rel{UsedFor, Causes} & 800 & 28 %& $\langle$\textit{reading, education}$\rangle$ 
\\
\rel{HasSubevent, Causes} & 636 & 70 %& $\langle$\textit{playing games, fun}$\rangle$ 
\\
\rel{HasSubev., HasPrereq.} & 628 & 90 %& $\langle$\textit{dream, sleep}$\rangle$ 
\\
\rel{HasPrereq., HasFirstSubev.} & 520 & 150 %& $\langle$\textit{act in play, learn script}$\rangle$  
\\
\rel{HasSubev., HasFirstSubev,} & 316 & 66 %& $\langle$\textit{attend classical concert, buy ticket}$\rangle$  
\\
\rel{UsedFor, HasSubev.} & 254 & 14 %& $\langle$\textit{having lunch, eating}$\rangle$ 
\\
\rel{HasSubev., Motiv.ByGoal} & 252 & 58 %& $\langle$\textit{pray, talk to god}$\rangle$ 
\\
\rel{HasSubevent, Other} & 164 & 86 %& $\langle$\textit{attend class, take notes}$\rangle$ 
\\
%%\rel{HasPrereq., Motiv.ByGoal} & 128 & 42 %& $\langle$\textit{diminish your own hunger, eat}$\rangle$ 
%%\\
%%\rel{UsedFor, HasPrereq.}& 116 & 4 %& $\langle$\textit{understanding something, learning}$\rangle$ 
%%\\
%%\rel{HasPrereq., Other} & 106 & 54 
%& $\langle$\textit{awake, open eyes}$\rangle$  
%%\\
%%\rel{HasFirstSubev., Other} & 102 & 48 %& $\langle$\textit{express how funny, laugh}$\rangle$  
%%\\
%%\rel{Desires, CapableOf} & 46 & 44 
%& $\langle$\textit{people, eat in groups}$\rangle$ 
%%\\
\hline
\end{tabular}
}
\caption{Frequency of most co-occurring relations in \textsc{Cn-Omcs-Cln} and \textsc{Cn-Omcs-14}.}
\label{table:amb}
\vspace{-0.1in}
\end{table}


==> tables/moreambigrelationexamples.tex <==
\begin{table*}
\centering
\begin{tabular}{ll|ll}
Relations  &  & Concept 1 & Concept 2\\
\hline
\textsc{Desires}&\textsc{AtLocation} & a cat & a warm bed\\
\textsc{Desires} &\textsc{CapableOf}&  cats & mice\\
\textsc{HasSubevent}&\textsc{Causes} &  walking in the rain & get wet\\
\textsc{HasSubevent} &\textsc{HasPrerequisite} &  take final exams & study\\
\textsc{UsedFor} &\textsc{CapableOf} &  Forklifts & lift heavy things\\
%\textsc{Desires} &\textsc{CapableOf} &  children & throw things\\
%\textsc{Desires} &\textsc{CapableOf}&  dogs & eat people\'s food\\

\end{tabular}
\caption{Pairs of concepts which are connected by multiple relations in ConceptNet}
\label{table:examples}
\end{table*}

==> tables/other.tex <==
\begin{table} [t]
\scalebox{0.8}{
\begin{center}
\begin{tabular}{|lll|}
\hline
\small\rel{MadeOf} & \small\rel{FormOf} & \small\rel{HasContext} \\
\small\rel{dbpedia} & \small\rel{DerivedFrom} & \small\rel{DefinedAs} \\
\small\rel{RelatedTo} & \small\rel{ObstructedBy} & \small\rel{HasLastSubev.} \\
\small\rel{Difference} & \small\rel{Synonym} & \small\rel{ExternalURL} \\
\small\rel{LocatedNear} & \small\small\rel{PartOf}  & \small\rel{InstanceOf}  \\
\small\rel{CreatedBy} & \small\rel{SymbolOf} & \small\rel{NotCapableOf} \\ 
\small\rel{NotUsedFor} & \small\rel{NotDesires} & \small\rel{NotHasProp.} \\
\hline

\end{tabular}
\end{center}
}
\caption{Relations contained in the \small\rel{Other} class.\footnote{\small\rel{EtymologicallyRelatedTo} occurs only once in our dataset and is not included in the table.}}
%(each$<$2000 instances).

\label{tbl:other}
\end{table} 



==> tables/relationset.tex <==
\begin{table}[t]
\small{
\scalebox{0.91}{
\begin{tabular}{@{}llll@{}ccl}
\toprule
\cn&\multicolumn{2}{c}{concept type}& \multicolumn{2}{c}{phrase type}& multiword concepts (in \%) & words per term (avg.) & multi-label instances (in \%) \\
relation& \textsc{arg$_1$} & \textsc{arg$_2$}& \textsc{arg$_1$} & \textsc{arg$_2$}&in \%\\ %& between relations\\
\midrule
\textsc{IsA} & \cellcolor{red!25}entity & \cellcolor{red!25}entity& NP & NP&0.49\\

\textsc{AtLocation} & \cellcolor{red!25}entity&\cellcolor{gray!25}location & NP & NP& 0.76\\
\textsc{HasProperty}& \cellcolor{red!25}entity& \cellcolor{yellow!25}property& NP & AP&0.49 \\
\textsc{Desires}& \cellcolor{red!25}entity & \cellcolor{red!25}entity & NP & NP&0.73\\
\textsc{UsedFor} & \cellcolor{red!25}entity & \cellcolor{cyan!25}event& NP & VP&0.78\\
%\textsc{R$_5$($c_1$,$c_2$) $\rightarrow$ \\%R$_6$($c_1$,$c_2$)}\\
\textsc{CapableOf}& \cellcolor{red!25}entity & \cellcolor{cyan!25}event& NP &VP&0.76 \\%&\textsc{R$_6$($c_1$,$c_2$) $\Diamond\hspace*{-2mm}\rightarrow$ R$_5$($c_1$,$c_2$)}\\
\textsc{HasSubevent}& \cellcolor{cyan!25}event & \cellcolor{cyan!25}event& VP &VP&0.81\\%&\textsc{R$_9$($c_1$,$c_2$) $\Diamond\hspace*{-2mm}\rightarrow$ R$_7$($c_1$,$c_2$)}\\
\textsc{HasPrerequisite}& \cellcolor{cyan!25}event & \cellcolor{cyan!25}event&VP&VP&0.84 \\%&\textsc{R$_8$($c_1$,$c_2$) $\Diamond\hspace*{-2mm}\rightarrow$ R$_9$($c_1$,$c_2$)}\\
\textsc{Causes} &\cellcolor{cyan!25}event & \cellcolor{cyan!25}event&VP& NP&0.74\\%& \textsc{R$_6$($c_1$,$c_2$), R$_9$($c_2$,$c_3$) $\Diamond\hspace*{-2mm}\rightarrow$ R$_9$($c_1$,$c_3$)}\\
\textsc{MotivatedByGoal} & \cellcolor{cyan!25}event & \cellcolor{cyan!25}event &VP&VP&0.89\\%& \textsc{R$_4$($c_1$,$c_2$), R$_8$($c_3$,$c_2$) $\Diamond\hspace*{-2mm}\rightarrow$ R$_{10}$(c$_3$,$c_2$)}\\
\bottomrule
\end{tabular}
}
\caption{Relations in \cn, concept and phrase types; multiword percentages (total: 0.76)
%($\Diamond$ indicates possibility)
%\\\rednote{@BK: you detected more connections between relations. please insert or add to caption
}
\label{tbl:CN14relations}
}
\vspace{-0.1in}
\end{table}

==> tables/relationset_new.tex <==
\begin{table*}[t]

\small{
\scalebox{0.99}{
\centering
\begin{tabular}{@{}llll@{}l|lll}
\toprule
 &\multicolumn{2}{c}{concept type}& \multicolumn{2}{c}{phrase type}& multiword & words per & multi-label \\%&  thres- & single tune 

relation& \textsc{arg$_1$} & \textsc{arg$_2$}& \textsc{arg$_1$} & \textsc{arg$_2$}&concepts (\%) & concept (avg) & relations (\%) \\ %& hold & improv.\\ 
\midrule

\textsc{UsedFor} & \cellcolor{red!40}entity & \cellcolor{yellow!35}event& NP & VP&0.64 (0.64) & 1.90 (1.95) &  ~3.25 ~~(4.41) %& 0.27 & 0
\\
\textsc{AtLocation} & \cellcolor{red!40}entity&\cellcolor{gray!25}location & NP & NP& 0.36 (0.35) & 1.43 (1.42) &  ~1.86 ~~(1.06) %& 0.04 & 2
\\
\textsc{HasSubevent}& \cellcolor{yellow!35}event & \cellcolor{orange!70}ev/entity& VP &V/NP&0.79 (0.80) & 2.20 (2.21) &  14.94 (11.02) %& 0.04 & 9
\\
\textsc{CapableOf}& \cellcolor{red!40}entity & \cellcolor{yellow!35}event& NP &VP&0.56 (0.58) & 1.83 (1.89) &  ~2.86 ~~(1.17) %&0.04 & 1
 \\
\textsc{HasPrerequisite}& \cellcolor{yellow!35}event & \cellcolor{yellow!35}event&VP&VP&0.78 (0.80) & 2.15 (2.23) &  13.70 ~(9.86) %& 0.08 & 2
 \\
\textsc{IsA} & \cellcolor{red!40}entity & \cellcolor{red!40}entity& NP & NP&0.43 (0.46) & 1.72 (1.78) &  ~1.70 ~~(1.17) %& 0.04 & 3
\\
\textsc{Causes} &\cellcolor{orange!70}ev/entity & \cellcolor{orange!70}ev/entity&V/NP& V/NP&0.72 (0.73) & 2.04 (2.10) &  ~4.18 ~~(12.47) %& 0.02 & 1
\\
\textsc{Motiv.ByGoal} & \cellcolor{yellow!35}event & \cellcolor{yellow!35}event &VP&VP&0.78 (0.79) & 2.16 (2.21) &  ~5.19 ~~(6.57) %& 0.31 & 0
\\
\textsc{HasProperty}& \cellcolor{red!40}entity& \cellcolor{cyan!25}property& NP & AP&0.40 (0.41) & 1.75 (1.80) &  ~0.62 ~~(1.31) %& 0.04 & 1
 \\
\textsc{ReceivesAction}& \cellcolor{red!40}entity& \cellcolor{yellow!35}event& NP & VP&0.56 (0.58) & 2.21 (2.24) &   ~0.15 ~~(0.18) %& 0.02 &0
 \\
\textsc{HasA} & \cellcolor{red!40}entity & \cellcolor{red!40}entity & NP & NP&0.55 (0.56) & 1.88 (1.96) &   ~0.46 ~~(1.07) %& 0.96 &2
\\
\textsc{CausesDesire} & \cellcolor{red!40}entity& \cellcolor{yellow!35}event& NP & VP&0.74 (0.74) & 2.09 (2.10) &  ~0.23 ~~(0.67) %& 0.76 &0
\\
\textsc{HasFirstSubev.} & \cellcolor{yellow!35}event & \cellcolor{orange!70}ev/entity& VP &V/NP&0.85 (0.84) & 2.30 (2.27) &  10.84 (36.26) %& 0.59 &1
\\
\textsc{Desires} & \cellcolor{red!40}entity & \cellcolor{yellow!35}ev/\cellcolor{orange!70}entity& VP &V/NP&0.40 (0.40) & 1.68 (1.68) &   ~2.01 ~~(2.79) %& 1.00 &5
\\
\hline
\textsc{Other} & / & / & / & / &0.53 (0.5) & 1.82 (1.81) &   ~9.52 ~~(7.18) %& 0.35 &0
\\
\textsc{Random} & / & / & / & / &0.55 (0.63) & 1.84 (1.97) &   / %& 0.02 &4
\\
All relations (OW)  & / & / & / & / & 0.60 () & 1.94 (x) &  ~4.77 ~~(x) %& 0.36 &2
\\
\bottomrule
\end{tabular}
}
\caption{Relations in \cn, concept types and phrase types (column 1-4); percentage of multiword-concepts and average number of words per concept (column 5-6); improvement of our \textsc{Ffnn} model when enhanced with \textsc{Rnn} for multiword representation (Open world-one class setting; in percentage points) (column 7); and percentage of co-occurences of relations with other relations (column 8). Numbers refer to \textsc{Cn-Omcs-2000}, numbers in brackets display statistics for \textsc{Cn-Omcs} (cleaned version).
%($\Diamond$ indicates possibility)
%\\\rednote{@BK: you detected more connections between relations. please insert or add to caption
}
\label{tbl:relations_statistics}
}
\vspace{-0.1in}
\end{table*}




==> tables/thresholds.tex <==
\begin{table}[th]
\centering
%\scalebox{.80}{
%\begin{tabular}{@{}lll||ll|ll|lll@{}}
\begin{tabular}{lllllllllllll}
\toprule


%Setting &  \multicolumn{2}{c}{Open World (1 Class)} &  \multicolumn{2}{c}{Open World (2 Classes)} &\multicolumn{3}{c}{Closed World} & \multicolumn{3}{c}{} \\
%\hline
%Model &  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}\\

%Setting &  \multicolumn{2}{c}{OW-1} &  \multicolumn{2}{c}{OW-2} & \multicolumn{2}{c}{CW} & \multicolumn{3}{c}{}\\
%\hline
%Model &  \scriptsize{FFNN} & \scriptsize{FFNN} &  \scriptsize{FFNN} & \scriptsize{FFNN} &  \scriptsize{FFNN} & \scriptsize{FFNN}\\
% &  & \scriptsize{+RNN}&  & \scriptsize{+RNN}&  & \scriptsize{+RNN}\\
%Relation         & \multicolumn{2}{c}{~~~~~~~~~+RNN} \\
%Relation \\
\hline \hline
\small{\rel{UsedFor}} & x & x & .06 & .27 & .88 & .92\\
\small{\rel{AtLocation}} & x & x & .92 & .04 & .90 & .90\\
\small{\rel{HasSubevent}} & x & x & .02 & .04 & .41 & .02\\
\small{\rel{CapableOf}} & x & x & .96 & .04 & .02 & .18\\
\small{\rel{HasPrerequisite}} & x & x & .02 & .08 & .98 & .10\\
\small{\rel{IsA}} & x & x & .88 & .04 & .67 & .51\\
\small{\rel{Causes}} & x & x & .73 & .02 & .10 & .27 \\
\small{\rel{Motiv.ByGoal}}& x & x & .02 & .31 & .14 & .96\\
\small{\rel{HasProperty}} & x & x & .90 & .04 & .98 & .98 \\
\small{\rel{ReceivesAction}} & x & x & .90 & .02 & .94 & .12\\
\small{\rel{HasA}} & x & x & .96 & .96 & .27 & .98\\
\small{\rel{CausesDesire}}& x & x & .90 & .76 & 1.0 & .98 \\
\small{\rel{HasFirstSubev.}} & x & x & .57 & .59 & .08 & .94\\
\small{\rel{Desires}} & x & x & 1.0 & 1.0 & 1.0 & 1.0 \\ \hline
\small{\rel{Other}} & - & - & .96 & .35 & - & -\\
\small{\rel{Random}} & - & - & .04 & .02 & - & -\\ 
\small{\rel{Other+Random}} & x & x & - & - & - & -\\ 
\hline \hline
Mutually Tuned & x & x & x & .36 & x & .95\\ \hline
\bottomrule
\end{tabular}
%}
\caption{Optimal thresholds when tuning  evaluation threshold separately for each relation on \textsc{Cn-Omcs-2000} with different settings and models.
OW-1 refers to the Open World Setting which includes one mixed Open World class (\rel{Other+Random}), OW-2 describes the Open World Setting which includes two Open World classes (\rel{Other} and \rel{Random} separately), and CW is the Closed World Setting.}%improvement when thresholds are tuned separately instead of mutually (\textsc{Ffnn-Rnn}), in percentage points (column 10). \rednote{MB: I'm not so sure about the last two columns and how to interpret them. If they are not expressive/interpretable we should maybe skip them?}

\label{tbl:thresholds}
\end{table}

==> tables/thresholds_new.tex <==
\begin{table}[th]
\centering

\scalebox{0.7}{
\begin{tabular}{lllllllllllll}
\toprule


%Setting &  \multicolumn{2}{c}{Open World (1 Class)} &  \multicolumn{2}{c}{Open World (2 Classes)} &\multicolumn{3}{c}{Closed World} & \multicolumn{3}{c}{} \\
%\hline
%Model &  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}\\

%Setting &  \multicolumn{2}{c}{OW-1} &  \multicolumn{2}{c}{OW-2} & \multicolumn{2}{c}{CW} & \multicolumn{3}{c}{}\\
%\hline
%Model &  \scriptsize{FFNN} & \scriptsize{FFNN} &  \scriptsize{FFNN} & \scriptsize{FFNN} &  \scriptsize{FFNN} & \scriptsize{FFNN}\\
% &  & \scriptsize{+RNN}&  & \scriptsize{+RNN}&  & \scriptsize{+RNN}\\
%Relation         & \multicolumn{2}{c}{~~~~~~~~~+RNN} \\
%Relation \\

Setting & OW-1 & &  OW-2 & & CW &  \\
Model &  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}&  FFNN & FFNN\small{+RNN}\\
\hline \hline
\small{\rel{UsedFor}} & .20 & .37 & .06 & .27 & .88 & .92\\
\small{\rel{AtLocation}} & .84 & .65 & .92 & .04 & .90 & .90\\
\small{\rel{HasSubevent}} & .04 & .12 & .02 & .04 & .41 & .02\\
\small{\rel{CapableOf}} & .04 & .24 & .96 & .04 & .02 & .18\\
\small{\rel{HasPrerequisite}} & .02 & .41 & .02 & .08 & .98 & .10\\
\small{\rel{IsA}} & .37 & .04 & .88 & .04 & .67 & .51\\
\small{\rel{Causes}} & .10 & .06 & .73 & .02 & .10 & .27 \\
\small{\rel{Motiv.ByGoal}}& .84 & .45 & .02 & .31 & .14 & .96\\
\small{\rel{HasProperty}} & .98 & .76 & .90 & .04 & .98 & .98 \\
\small{\rel{ReceivesAction}} & .16 & .08 & .90 & .02 & .94 & .12\\
\small{\rel{HasA}} & .94 & .90 & .96 & .96 & .27 & .98\\
\small{\rel{CausesDesire}}& .96 & .98 & .90 & .76 & 1.0 & .98 \\
\small{\rel{HasFirstSubev.}} & .78 & .78 & .57 & .59 & .08 & .94\\
\small{\rel{Desires}} & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\ \hline
\small{\rel{Other}} & - & - & .96 & .35 & - & -\\
\small{\rel{Random}} & .02 & .02 & .04 & .02 & - & -\\ 
\hline \hline
Mutually Tuned & .60 & .84 & .75 & .36 & .50 & .95\\ \hline
\bottomrule
\end{tabular}
}
\caption{\rednote{Table will probably be omitted/moved to supplement}. Optimal thresholds when tuning  evaluation threshold separately for each relation on \textsc{Cn-Omcs-2000} with different settings and models.
OW-1=Open World Setting which includes one Open World class (\rel{Random}), OW-2 d=Open World Setting which includes two Open World classes (\rel{Other} and \rel{Random} separately), CW=Closed World Setting.}%improvement when thresholds are tuned separately instead of mutually (\textsc{Ffnn-Rnn}), in percentage points (column 10). \rednote{MB: I'm not so sure about the last two columns and how to interpret them. If they are not expressive/interpretable we should maybe skip them?}

\label{tbl:thresholds}
\end{table}
